Bandits Meet Mechanism Design to Combat Clickbait in Online Recommendation

We study a strategic variant of the multi-armed bandit problem, which we coin the strategic click-bandit. This model is motivated by applications in online recommendation where the choice of recommended items depends on both the click-through rates and the post-click rewards. Like in classical bandits, rewards follow a fixed unknown distribution. However, we assume that the click-rate of each arm is chosen strategically by the arm (e.g., a host on Airbnb) in order to maximize the number of times it gets clicked. The algorithm designer does not know the post-click rewards nor the arms' actions (i.e., strategically chosen click-rates) in advance, and must learn both values over time. To solve this problem, we design an incentive-aware learning algorithm, UCB-S, which achieves two goals simultaneously: (a) incentivizing desirable arm behavior under uncertainty; (b) minimizing regret by learning unknown parameters. We characterize all approximate Nash equilibria among arms under UCB-S and show a $\tilde{\mathcal{O}} (\sqrt{KT})$ regret bound uniformly in every equilibrium. We also show that incentive-unaware algorithms generally fail to achieve low regret in the strategic click-bandit. Finally, we support our theoretical results by simulations of strategic arm behavior which confirm the effectiveness and robustness of our proposed incentive design.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/mnl_multi_slot.tex <==

\section{Extension: MNL Multi-Slot}

\SetAlgorithmName{Model}{}{}
\RestyleAlgo{boxruled}
\SetAlgoLined
\LinesNumbered
\begin{algorithm}[ht]
  \caption{MNL Multi-Slot Recommendations}
  Principal chooses an algorithm $M$, which is shared with all agents \\
  Agents decide on strategies $(\s_1, \dots, \s_K) \in [0,1]^K$ (unknown to $M$)\\
  \For{$t = 1, \dots, T$}{
  Mechanism $M$ selects subset $S_t \subseteq [K]$ of size $|S_t| = m$ \\
  Agent $i_t \in S_t \cup \{0\}$ receives a click, where each $i \in S_t \cup \{0\}$ is clicked with probability $$\P (c_t = i \mid S_t \cup \{0\}) = \frac{s_i}{s_0 + \sum_{j \in S_t} s_j}. $$ \\
  $M$ observes noisy post-click reward $r_{t, i} = \mu_i + \eta_t$, where $\eta_t$ is sub-Gaussian noise. 
%   If $i_t$ is clicked, a noisy post-click reward $r_{i_t}^t = \mu_{i_t} + \eta_t$ is observed, where $\eta_t$ is sub-Gaussian noise. 
%   If the item is clicked ($c^t_{i_t} = 1$), the mechanism observes a post-click reward $r_{i_t}^t := \mu_{i_t} + \eta_t$, where $\eta_t$ is sub-Gaussian noise.
  } 
\end{algorithm}


\subsection{Regret}

\begin{align*}
    R_T(M, \bsigma) := \E_{\bs \sim \bsigma} \left[ \sum_{t=1}^T \sum_{i^* \in S^*} u\big(s(\mu_{i^*}), \mu_{i^*}\big) - \sum_{i \in S_t} u(\s_i, \mu_i) \right]
\end{align*}

% \begin{align*}
    % R_T(M, \bsigma) :=  \sum_{t=1}^T \E [u(S^*) \mid \bs \sim \bsigma^*] -  \E [u(S_t) \mid \bs \sim \bsigma]
% \end{align*}



\subsection{Algorithm}

\SetAlgorithmName{Mechanism}{}{}
\RestyleAlgo{ruled}% Change from the 'boxed' style to 'ruled' 
\begin{algorithm}[H]
\caption{MNL-UCB with Screening (MNL-UCBS)}
\textbf{initialize:} $A_0 = [K]$, $\ell = 1$ \\ 
\For{$t=1,\dots, T$}{
Play $S_\ell = \argmax_{S \subseteq A_{\ell-1}} \sum_{i \in S} \overline \mu_i^{\ell-1}$ \\ 
Observe click-event $c_t = i_t$ and post-click reward $r_{t, i_t}$ \\
\If{$c_t = 0$}{
$\ell \leftarrow \ell + 1$ \\
update $\hat s_i^\ell$ \\
update $\hat \mu_i^\ell$ \\
$A_\ell \leftarrow A_{\ell-1} \setminus \{i \in [K] \colon \overline \s_{i}^\ell  < \min_{\mu \in [\underline{\mu}^\ell_{i}, \overline \mu_{i}^\ell]} \s(\mu) \ \textnormal{ or } \ \underline \s_{i}^\ell >  \max_{\mu \in [\underline{\mu}^\ell_{i}, \overline \mu_{i}^\ell]} \s(\mu)\}$ 
}
\Else{
$\mathcal{E}_\ell \leftarrow \mathcal{E}_{\ell} \cup \{t\}$}
}
\end{algorithm}

==> sections/motivation_figure.tex <==
% \begin{tikzpicture}
% \draw [draw=white] (1, 3.5) rectangle (5, 4) node[align=left, pos=.5]{Strategically Chosen \\ Headline \& Thumbnail};

% \draw (0,1.5) node{Arm $1$};
% \draw [draw=black] (1, 0) rectangle (5,1) node[pos=.5]{click-rate $\s_1$};% lower
% \draw [draw=black] (1, 1) rectangle (5,3) node[pos=.5]{\includegraphics[scale=0.2]{sections/figures/black_hole.png}};% upper


% \end{tikzpicture}

% \vspace{2cm}

% \begin{tikzpicture}
% \draw [draw=white] (1, 3.5) rectangle (5, 4) node[align=left, pos=.5]{Strategically Chosen \\ Headline \& Thumbnail};

% \draw (0,1.5) node{Arm $1$};
% \draw [draw=black] (1, 0) rectangle (5,1) node[pos=.5]{click-rate $\s_1$};% lower
% \draw [draw=black] (1, 1) rectangle (5,3) node[align=left, pos=.5]{WARNING: Supermassive \\ black hole heading \\ Earth's way at 110KM \\ per SECOND!};% upper


% \end{tikzpicture}




% \vspace{2cm}

% \begin{tikzpicture}
% \draw [draw=white] (1, 3.5) rectangle (5, 4) node[align=left, pos=.5]{Strategically Chosen \\ Headline \& Thumbnail};

% \draw (0,1.5) node{Arm $1$};
% \draw [draw=white] (1, 0) rectangle (5,1) node[pos=.5]{click-rate $\s_1$};% lower
% \draw (3, 2) node{\includegraphics[scale=.25]{sections/figures/world_end.png}};% upper


% \end{tikzpicture}

==> sections/old_notes/old_lower_bound.tex <==

- 
\newpage

\subsection{Lower Bound Proofs and Notes}



\subsection{Proof of Theorem~\ref{thm:lower_boun\s_known}}

\paragraph{Overview.} We prove Theorem~\ref{thm:lower_bound_known} by arguing that for any mechanism $M$ there always exists a problem instance such that for any Nash equilibria $\bs \in \NE(M)$, we have for $\s_{i^*} \in \supp(\sigma_{i^*})$ that $\s_{i^*} = \s(\mu_{i^*}) + \Omega(\frac{1}{\sqrt{T}})$, where $i^* := \argmax_{i \in [K]} \mu_i$ is the optimal arm. When choosing a problem instance $(\mu_1, \dots, \mu_K)$ with constant optimality gap, e.g., $\Delta_i \geq 1/2$ for all $i \neq i^*$, this implies a regret lower bound of $R_T(M, \bs) \geq T \cdot \Omega(\frac{1}{\sqrt{T}}) = \Omega(\sqrt{T})$.


\subsubsection{Information-Theoretic Preliminaries} 

We let $\KL(\P_1, \P_2)$ denote the KL-divergence (or relative entropy) between two probability measures $\P_1$ and $\P_2$. As a special case, we let $\kl(p, q)$ denote the KL-divergence between two Bernoulli distributions with means $\Bern(p)$ and $\Bern(q)$.  

A standard result from information theory is the the following divergence decomposition (e.g., \cite{lattimore2020bandit}). 
\begin{lemma}
    Let $P_i$ be the distribution associated with strategy $\s_i$. In our case, $P_i$ is a Bernoulli distribution with mean $\s_i$. 
    \begin{align}
    \sum_{i=1}^K \E_{M, \bs} [n_T(i)] \, \KL (P_i, P_i^\prime) = \KL(\P_{M, \bs}, \P_{M, \bs^\prime}).   
    \end{align}
    
\end{lemma} 

A very useful addition to the above divergence decomposition is a lower bound on $\KL(\P_\bs , \P_{\bs^\prime})$, which can be derived from the data-processing inequality. 

\begin{lemma}[\cite{garivier2019explore}]\label{lemma:garivier}
    
    \begin{align}
    \sum_{i=1}^K \E_{M, \bs} [n_T(i)] \, \KL (P_i, P_i^\prime) = \KL(\P_{M, \bs}, \P_{M, \bs^\prime}) \geq \kl (\E_{M, \bs} [Z], \E_{M, \bs^\prime} [Z]). 
    \end{align}
\end{lemma}


\subsubsection{Lower Bound on \texorpdfstring{$\E_{M, \bs} [n_T(i^*)]$ for any $M$ with $R_T(M, \bs^\prime) = O(\sqrt{T})$}{...}} 

Consider a problem instance $\mu_1, \dots, \mu_K$ such that $\Delta_i \geq 1/2$ and $\s(\mu_{i^*})$ is bounded away from $0$ and $1$. The specific value of $\s(\mu_{i^*})$ will not matter and w.l.o.g.\ let us assume $\s(\mu_{i^*}) = 1/2$. 

Let $M$ be any mechanism with $R_T(M, \bs) = o(\sqrt{T})$ for all $\bs \in \NE(M)$. A necessary condition for this to hold is that $\E_{d \sim \sigma_{i^*}}[d] = \s(\mu_{i^*}) \pm o(\frac{1}{\sqrt{T}})$ as well as $\E_{M, \bs} [n_T(i^*)] \geq T - o(\sqrt{T})$. 

W.l.o.g.\ assume $\sigma_{i^*}= \mathrm{Dirac}(\s(\mu_{i^*}))$ and write $\bs = (\sigma_1, \dots, \s(\mu_{i^*}), \dots, \sigma_K)$. Define $\bs_\varepsilon := (\sigma_1, \dots, \s(\mu_{i^*}) + \varepsilon, \dots, \sigma_K)$. 
We let $\P := \P_{M, \bs}$ denote the probability measure under $\bs$ and $\P_\varepsilon := \P_{M, \bs_\varepsilon}$ the probability measure under $\bs_\varepsilon$. 

Our goal is to prove that $\E_\varepsilon [n_T(i^*)] \geq T - O(\sqrt{T})$. To this end, suppose that $\frac{\E_{\varepsilon} [n_T(i^*)]}{T} \leq 1- \sqrt{\frac{c_1}{T}}$ for all $c_1 > 0$. Applying Lemma~\ref{lemma:garivier} to $\P$ and $\P_\varepsilon$, we obtain (with $Z=n_T(i^*)/T$)
\begin{align}
    \E_\varepsilon [n_T(i^*)] \, \kl (\s(\mu_{i^*})+ \varepsilon, \s(\mu_{i^*})) \geq \kl \left( \frac{\E_\varepsilon [n_T(i^*)]}{T}, \frac{\E [n_T(i^*)]}{T} \right),
\end{align}
where we used that $\sigma$ and $\sigma_\varepsilon$ coincide for all $i \neq i^*$, i.e.\ their relative entropy is zero. We now use that $\frac{\E[n_T(i^*)]}{T} \geq 1 - o(\frac{1}{\sqrt{T}}) \geq  1 - \sqrt{\frac{c_2}{T}}$ for some constant $c_2 > 0$, so that 
\begin{align}
    \kl \left( \frac{\E_\varepsilon [n_T(i^*)]}{T}, \frac{\E [n_T(i^*)]}{T} \right) \geq \kl \left( \frac{\E_\varepsilon [n_T(i^*)]}{T}, 1- \sqrt{\frac{c_2}{T}} \right) \geq  \frac{1}{2(1-\sqrt{\frac{c_2}{T}})} \left( \frac{\E_\varepsilon [n_T(i^*)]}{T} -  \left(1- \sqrt{\frac{c_2}{T}} \right) \right)^2, 
\end{align}
where we used the refined Pinsker's inequality for Bernoulli distributions: $\kl (p, q ) \geq \frac{1}{2q}(p-q)^2$ for $p \leq q$. We can upper bound the left hand side again using the assumption that $\frac{\E_{\varepsilon} [n_T(i^*)]}{T} \leq 1- \sqrt{\frac{c_1}{T}}$ for all $c_1 > 0$. This yields
\begin{align}
    T \left(1- \sqrt{\frac{c_1}{\sqrt{T}}}\right)  \kl (\s(\mu_{i^*}+\varepsilon, \s(\mu_{i^*})) \geq \frac{1}{2(1- \sqrt{\frac{c_2}{T}})} \left(  \left(1- \sqrt{\frac{c_2}{T}} \right) - \frac{\E_\varepsilon [n_T(i^*)]}{T} \right)^2. 
\end{align}
Taking the square-root and reordering, we get for $c_1 > c_2$:
\begin{align}
     \frac{E_\varepsilon[n_T(i^*)]}{T} \geq 1- \sqrt{\frac{c_2}{\sqrt{T}}} - \sqrt{2T \kl(\s(\mu_{i^*})+\varepsilon, \s(\mu_{i^*})}) \left(1- \sqrt{\frac{c_1}{T}}\right). 
\end{align}
We now use that for $\s(\mu_{i^*}) = 1/2$, we have $\kl(\s(\mu_{i^*}) + \varepsilon, \s(\mu_{i^*})) \leq 2 \varepsilon^2$ and choose $\varepsilon = \sqrt{\frac{c_3}{T}}$ for some $c_3 > 0$. This gives 
\begin{align}
    \E_\varepsilon[n_T(i^*)] \geq T - \sqrt{c_2 T}  - 2 c_3 \sqrt{T} - 2c_3 \sqrt{c_1} = T- O(\sqrt{T}).
\end{align}
Note that we can choose $c_3$ as close to zero as we want, so that essentially $\E_\varepsilon [n_T(i^*)] \geq T - \sqrt{c_2 T}$. 


% To derive lower bounds here is a bit more intricate than in the MAB problem, since the mechanisms influence the problem instances by incentivizing certain strategies. As a result, a good mechanism does not have to achieve low regret under all arm strategies, but only specifically for the incentivized strategies, i.e., the Nash equilibria given under the mechanism. 






\subsection{Some thoughts}

\begin{lemma}[Bretagnolle–Huber inequality]
    Let $P$ and $Q$ be probability measures on the same probability space $(\Omega, \mathcal{F})$, and let $A \in \mathcal{F}$ be an arbitrary event. Then, 
    \begin{align}
        P(A) + Q(A^c) \geq \frac{1}{2} \exp (- D(P, Q)),
    \end{align}
    where $D(P, Q)$ denotes the KL-divergence.
\end{lemma}
Note that the KL-divergence of two Bernoulli distributions with parameters $d$ and $d'$ is lower bounded by $D(d, d') \geq \frac{(d-d')^2}{d'(1-d')}$. 


Fix some mechanism $M$ and let $\P_{d_{i^*}}$ denote the probability measure under mechanism $M$ and strategy $d_{i^*}$. Applying the above lemma to our case, we can write
\begin{align}
    \P_{d(\mu_{i^*})} \left( n_T(i^*) \leq  \frac{T}{2}\right) + \P_{d_{i^*}} \left( n_T(i^*) >  \frac{T}{2}\right) \geq \frac{1}{2} \exp \big(-D(d(\mu_{i^*}), d_{i^*}) \big). 
\end{align}

% For any mechanism $M$ with $R_T(M, \bs)) = O(\sqrt{T})$ for all $\bs \in \NE(M)$, ..  


% \vspace{1cm}

\begin{proof}[Proof Idea]
There is an inherent tension between the allocations that an arm receives and how close their strategies $d$ are to the desired strategy $d(\mu)$ (at least when deploying a screening rule as we did in UCB-S). Any mechanism can promise to an arm at most $T$ selections in total (even an oracle that knows $i^*$ can only select the best arm at most $T$ times). \emph{With high confidence}, we can only detect a deviation $d- d(\mu)$ after order $\log(T) / (d-d(\mu))^2$ many selections. Hence, if any arm can expect at most $T$ selections, they can choose the largest $d$ so that $\log(T) / (d-d(\mu))^2 \geq T$, i.e.\ the largest $d$ so that $d-d(\mu) \leq \sqrt{{\log(T)}/{T}}$. Hence, any arm will deviate always at least $\sqrt{\log(T) / T}$ from the desired strategy $d(\mu)$. For any of our selections, we therefore suffer at least this amount of instantaneous regret so that in total the regret of any mechanism is lower bounded by $\Omega(T \cdot \sqrt{\log(T)/T}) = \Omega(\sqrt{T \log(T)})$. 
\end{proof}



\newpage 

\section{Reverse Chernoff Bound Ideas for a Lower Bound Proof}

\begin{lemma}[Chernoff Bound]
Let $X_1, \dots, X_T$ be i.i.d.\ $\mathrm{Bern}(p)$ with $p \in (0, 1]$ and let $X := \frac{1}{T} \sum_{k=1}^T X_k$. For every $c > 0$, we have 
\begin{align}
    \P \left( X \geq p + \frac{c}{\sqrt{T}}\right) \leq \exp(- c^2 / 3 p).  
\end{align}
In particular, for $c = \sqrt{\log(1/\delta)}$, we get 
\begin{align}
    \P \left( X \geq p + \sqrt{\frac{\log(1/\delta)}{{T}}} \right) \leq O(\delta).
\end{align}
\end{lemma}
We state a reverse Chernoff bound for the specific case of $p=1/2$. There exists a more general version, see \cite{klein1999}, Lemma 5.2. 
\begin{lemma}[Reverse Chernoff Bound]
Let $X_1, \dots, X_T$ be i.i.d.\ $\mathrm{Bern}(p)$ with $p = 1/2$ and $X := \frac{1}{T} \sum_{k=1}^T X_k$. For any $0 < c < \frac{\sqrt{T}}{2}$, we have
\begin{align*}
    \P \left(X \geq p + \frac{c}{\sqrt{T}}\right) \geq \exp(-18 c^2). 
\end{align*}
For the typical $c = \sqrt{\log(1/\delta)}$ factor, we then have 
\begin{align*}
    \P\left( X \geq p + \sqrt{\frac{\log(1/\delta)}{{T}}} \right) \geq \Omega(\delta). 
\end{align*}
\end{lemma}

Let us now try to apply these bounds to our problem. W.l.o.g.\ let $d(\mu_{i^*}) = 1/2$ as we can design such a problem instance by choosing an appropriate $\mu_{i^*}$.\footnote{The function $d(\mu)$ is assumed be Lipschitz and therefore continuous.} Let $c^t_{i^*} \sim \mathrm{Bern}(d(\mu_{i^*}))$ under probability measure $\P$ and let $\hat d^t_{i^*} = \frac{1}{t} \sum_{k=1}^t c^k_{i^*}$ for $t \in [T]$. We then have 
\begin{align}
    \P \left( \hat d^T_{i^*} \geq d(\mu_{i^*}) + \sqrt{\frac{\log(1/\delta}{T}} \right) \geq \Omega(\delta).
\end{align} 
That is, the probability of the average $\hat d^T_{i^*}$ of $d(\mu_{i^*})$ exceeding $d(\mu_{i^*}) + \sqrt{\frac{\log(1/\delta)}{T}}$ is at least $\Omega(\delta)$. 

Now, let $\P_\varepsilon$ denote the probability measure under which $c^t_{i^*} \sim \mathrm{Bern}(d(\mu_{i^*})+\varepsilon)$. Let $\varepsilon := \sqrt{\frac{z}{T}}$ for some constant $z < \log(1/\delta) / 2$ to be chosen later. Using a standard Chernoff bound, we obtain 
\begin{align}
    & \P_\varepsilon \left( \hat d^T_{i^*} \geq d(\mu_{i^*}) + \sqrt{\frac{\log(1/\delta)}{T}} \right) \\
    & = \P_\varepsilon \left( \hat d^T_{i^*} \geq \left( d(\mu_{i^*}) + \varepsilon \right) + \left( \sqrt{\frac{\log(1/\delta)}{T}} - \varepsilon\right)\right) \\
    & \leq \exp\left( - \left( \sqrt{\frac{\log(1/\delta)}{T}} - \sqrt{\frac{z}{T}} \right)^2 / 3 \right) \\ 
    & \leq O(\delta) \cdot O\big(\left(1/\delta \right)^{z \alpha} \big) = O(\delta^{1-z \alpha}). 
\end{align}
for any $\alpha > 0$. This should follow from the fact that $\exp(\sqrt{\log(x)}) = O(x^\alpha)$ for all $\alpha > 0$. 


\textbf{To briefly summarise the above:} For $\varepsilon = \sqrt{z /T}$ and any $z, \alpha, \delta > 0$, we have shown
\begin{align}
    & \P \left( \hat d^T_{i^*} \geq d(\mu_{i^*}) + \sqrt{\frac{\log(1/\delta)}{T}} \right) \geq \Omega(\delta) \\
    & \P_\varepsilon \left(\hat d^T_{i^*} \geq d(\mu_{i^*}) + \sqrt{\frac{\log(1/\delta)}{T}} \right) \leq O(\delta^{1-z\alpha}). 
\end{align}



==> sections/old_notes/old_notes.tex <==


\section{Models}
\paragraph{Single-Slot Recommendations.} There are $K$ agents (i.e., the \emph{arms}). The game is played repeatedly for $T$ rounds. At any round $t = 1, \cdots, T$, the following happens in order:
\begin{enumerate}
    \item  The platform picks $i_t \in [K]$.
    \item Item $i_t$ is clicked with probability $d_{i_t} \in [0, 1]$, which is the ``marketing value'' of agent $i_t$'s item ($i_t$ will not be clicked with probability $1 - d_{i_t}$)
    \item Given that the arm is clicked, then the follow-up true reward $r_{i_t}^t$ from agent $i_t$ at time $t$ is realized. Assume $r_{i} \in [0,1]$  is drawn from an arbitrary distribution with mean $\mu_i$. 
\end{enumerate}

The objective of arm $i$, who knows their own $\mu_i$, is to find a marketing value $d_i$ at the very beginning of the game, in order to maximize the total arm surplus, defined as
\begin{equation}
    S_i(d_i, d_{-i}, \pi) = \E \left[ \sum_{t = 1}^T \mathbb{I}(i_t = i) d_{i_t} \mu_{i_t} \right]   
    \end{equation}
where the expectation is taken over the platform's selections and the environment's randomness. 
In the following, we typically assume that the arms play a Nash equilibrium of the game between arms defined by values $\mu_1, \dots, \mu_K$, the platform's selection and payment rule, and the surplus function $S$. 

\paragraph{Objectives.}  
The benign platform wants to maximizes the total welfare  $\sum_{t=1}^T  [d_{i_t} \mu_{i_t} - \pen(d_{i_t}, \mu_{i_t}) ]$, 
where the penalty function $\pen \colon [0,1] \times [0,1] \to \mathbb{R}$ is assumed to be $L$-Lipschitz w.r.t.\ the $\ell_1$-norm. An example of $\pen$ could be $\pen (d, \mu) = \lambda(d - \mu )^2$. For convenience, we define the welfare function $u(d, \mu) := d \mu - \pen(d, \mu)$. We will be interested in minimizing the expected regret 
\begin{equation}
    R(T) = \E \left[ \sum_{t=1}^T  u(d^*(\mu_{i^*}), \mu_{i^*}) - u(d_{i_t}, \mu_{i_t}) \right].
\end{equation}
For this notion of regret to be well-defined, we must state the objective of the arms. 
\hf{The benchmark might be always pull $i^* = \arg \max_i \mu_i$ and set $d_i = \mu_i (1+ \frac{1}{2\lambda}) = d^*(\mu_i)$. Assuming only Lipchitze continuity (notably, no monotonicity), then running UCB, we use $ \max_{\mu_i \in (\underline{\mu_i}, \bar{\mu_i} )}d^*(\mu_i) $ for the confidence bound of $d_i$   }

% So the first research question is  
\begin{question}
Is it possible for the platform to achieve good welfare with just the selection rule (i.e., always setting $m_i = 0$)? (Or can we show an example if we don't use payment, it's definitely bad for the platform?)
\end{question}
% The above objective does not have payment yet, so the only pay the RS can coordinate arms' selfish behavior is by designing the selection rule. 


\begin{question}
If we introduce payment $m_i(\mathcal{H}_i^T)$, can we improve the welfare, compared to the best welfare achievable without using payment?
\end{question} 


\paragraph{Notation.} We let the best arm w.r.t.\ the true reward denote $i^* = \argmax_i \mu_i$ and for convenience assume that this index is unique. We define the function $d^* \colon [0,1] \to [0,1]$ that maps from true rewards to desired marketing values as $d^*(\mu) = \argmax_{d\in [0,1]} u(d, \mu)$. % Note that $\pen(d, \mu)$ is Lipschitz so that $u(d, \mu)$ is differentiable in $d$ almost everywhere.  
Let $\bd = (d_1, \dots, d_k)$ and $\bmu = (\mu_1, \dots, \mu_K)$. 


\section{Algorithms (no payments)}


Let $n_t(d, i)$ be the number of times up to round $t$ that arm $i$ was selected by the platform. Let $n_t(\mu, i)$ be the number of times follow-up rewards were observed up to round $t$. Let $\hat d^t_i$ be the observed average click-rate and $\hat \mu^t_i$ the observed average follow-up reward. We construct lower and upper confidence bounds as $\underline d_i^t = \hat d_i^t - \sqrt{{2\log(T)}/{n_{t}(d, i)}}$ and $\overline \mu_i^t = \hat \mu_i^t + \sqrt{{2\log(T)}/{n_{t}(\mu, i)}}$. 


\begin{algorithm}[H]
\caption{UCB with Screening (UCB-S)}
\label{alg:ucb_screening}
\begin{algorithmic}[1] 
\STATE \textbf{initialize} $A_0 = [K]$ 

\FOR{$t =1, \dots, T$}
\STATE $A_t \leftarrow A_{t-1} \setminus \{i \in [K] \colon \underline d_i^t > \max_{\mu \in [\underline{\mu}^t_i, \overline \mu_i^t]} d^*(\mu)\}$ 
\STATE Play $i_t \in \argmax_{i \in A_t} \overline \mu_i^t$ 
\ENDFOR
% \STATE [Need to clarify what happens if $A_t = \emptyset$]
\end{algorithmic}
\end{algorithm} 

If we play UCB with payoffs $\mu$ or $d \mu$, it's clear that this doesn't work. 

Why does the following standard UCB approach does not work?  
\begin{algorithm}[H] \caption{UCB}
\begin{algorithmic}[1] 
\FOR{$t =1, \dots, T$}
\STATE Play $i_t \in \argmax_{i \in [K]} \overline u_i^t$ with $$\overline u_i^t = \max_{d \in [\underline d_i^t, \overline d_i^t]} \max_{\mu \in [\underline \mu_i^t, \overline \mu_i^t]} u_i(d, \mu)$$ 
\ENDFOR
\end{algorithmic}
\end{algorithm} 



\section{Analysis} 

\subsection{Characterizing Nash Equilibria under UCB-S}
The trickiest part of analysing the regret of a mechanism $\pi$ is characterizing the set of Nash equilibria for the arms. Recall that the game for the arms is defined by the tuple $G = (S, \bmu, \pi)$, i.e.\ the arms' surplus function $S$, the platform's selection rule $\pi$, and the true values $\bmu$. 
Here, the dependence on $\pi$ is the most challenging as the platform is uncertain about $\bd$ as well as $\bmu$. 



\begin{lemma}
Under UCB-S, any (pure) Nash equilibrium $(d_1, \dots, d_K)$ satisfies 
\begin{enumerate}
    \item[(i)]  $d_{i} \geq d^*(\mu_{i}) - 1/T^2$ for all $i \in [K]$ 
    \item[(ii)] $|d_{i^*} - d^*(\mu_{i^*})| \leq \sqrt{{c \log(T)}/{\E [n_T(i^*) | \bd]}}$ for some universal constant $c \geq 0$
\end{enumerate}
\end{lemma}
\hf{Conjecture: at any equilibrium, any agent $i$ who uses a $d_{i} \geq d^*(\mu_{i}) + \sqrt{{c \log(T)}/{\E [n_T(i^*) | \bd]}}$ cannot be pulled by more than $\log^2(T)$ times (since it will be screened out after $\sqrt{{c \log(T)}/{\E [n_T(i^*) | \bd]}}$ rounds). }
\begin{proof}
To get a foot into the door, let's first work under the following simplifying assumption: Every time $i_t$ is selected a follow-up reward $r_{i_t}^t$ with $\E [r_{i_t}^t] = \mu_{i_t}$ is observed (no matter the click-event), i.e.\ $n_t(d, i) = n_t(\mu, i)$. 

\emph{[In Progress]}
(i): 
% We first note that, given $i \in A_t$ for all $t \in [T]$, the surplus $S_i (d_i, d_{-i})$ is monotonically increasing as $d_i \to 1$ for all $d_{-i}$. Let $d_i = d^*(\mu_i)$ \tkb{This is actually not clear.}. 
Applying Hoeffding's inequality twice, it follows that with probability $1-1/T^2$ we have
\begin{align*}
    \underline d_i^t \leq d_i = d^*(\mu) \leq \max_{\mu' \in [\underline \mu_i^t, \overline \mu_i^t]} d^*(\mu')
\end{align*}
for all $t \in [T]$. Hence, $i \in A_t$ for all $t \in [T]$ with probability $1-1/T^2$. Let $\mathcal{E}_i = \{ i \in A_t \, \forall t \in [T]\}$. 
Suppose that $d_i < d^*(\mu_i) - d^*(\mu_i) / T^2$. For any $d_{-i}$, we then have 
\begin{align*}
    S_i(d^*(\mu_i), d_{-i}) & = \E \left[ n_T(i) \mid (d^*(\mu_i), d_{-i}) \right] d^*(\mu_i) \mu_i \\ 
    & \geq \E \left[ n_T(i) \mid (d^*(\mu_i), d_{-i}), \mathcal{E}_i \right] d^*(\mu_i) \mu_i (1- 1/T^2)  \\
    & > \E \left[ n_T(i) \mid (d^*(\mu_i), d_{-i}), \mathcal{E}_i \right] d_i \mu_i \\ 
    & = \E \left[ n_T(i) \mid (d_i, d_{-i}), \mathcal{E}_i \right] d_i \mu_i \\
    & \geq \E \left[ n_T(i) \mid (d_i, d_{-i})\right] d_i \mu_i = S_i (d_i, d_{-i}),
\end{align*}
where in the second last line we used that  $\E \left[ n_T(i) \mid (d_i, d_{-i}), \mathcal{E}_i \right] = \E \left[ n_T(i) \mid (d'_i, d_{-i}), \mathcal{E}_i\right]$ for all choices of $d_i, d'_i \in [0,1]$ and $d_{-i}\in [0,1]^{K-1}$. This means that $d^*(\mu_i)$ strictly dominates every $d_i < d^*(\mu_i) - 1/T^2$. Hence, any Nash equilibrium $\bd = (d_i, d_{-i})$ must satisfy $d_i \geq d^*(\mu_i) - 1/T^2$ for all $i \in [T]$. 



\vspace{1cm}

$$S_{i^*} ( d(\mu_{i^*}) + \varepsilon, d_{-i^*}) = O\left( \left( \frac{\log(T)}{\varepsilon^2} \wedge \E_{\textnormal{UCB}} [n_T(i^*)] \right) (d(\mu_{i^*}) + \varepsilon) \mu_{i^*} \right)$$
The maximum of this expression is achieved when $\log(T) / \varepsilon^2$ roughly equals $\E_{\textnormal{UCB}}[n_T(i^*)]$.
This means that $\varepsilon = O\left(\sqrt{\frac{\log(T)}{\E_{\textnormal{UCB}}[n_T(i^*)]}}\right)$. 


$\E_{\textnormal{UCB}}[n_T(i^*)]$ refers to the number of times $i^*$ is played when $i^*$ would not be eliminated. % when $d_{i^*} = d(\mu_{i^*})$. 
$\E_{\bd}[n_T(i^*)]$ w.r.t.\ the NE $\bd$ may be slightly smaller, but ... 


% We use the following properties of $n_T(i)$: 
% \begin{enumerate}
%     \item[(a)] We have $\E \left[ n_T(i) \mid (d_i, d_{-i}) \right] \leq \E \left[ n_T(i) \mid (d'_i, d_{-i}) \right]$ for all $d'_i \leq d_i$ and for all $d_{-i}$. 
%     \item[(b)] Let $\mathcal{E}_i = \{ i \in A_t \, \forall t \in [T]\}$. We have $\E \left[ n_T(i) \mid (d_i, d_{-i}), \mathcal{E}_i \right] = \E \left[ n_T(i) \mid (d'_i, d_{-i}), \mathcal{E}_i\right]$ for all $d_i, d'_i, d_{-i}$.
% \end{enumerate}

(ii): 
% The Chernoff bound is tight up to constant factors in the exponent for Bernoulli noise. Similarly, the Hoeffding bound is tight up to constant factors in the exponent for sub-Gaussian noise. 



\end{proof}

\subsection{Conjectured Regret Upper Bound} 

\begin{conjecture}
Let $\Delta_{\mu, i} := \mu_{i^*} - \mu_i$. Suppose that the arms play any Nash equilibrium under UCB-S. 
Then, the regret of UCB-S is upper bounded by 
\begin{equation*}
    R(T) = O \Big( \underbrace{ L \sqrt{T \log(T)}}_{\text{exploitation due to estimation}} + \underbrace{\sum_{i \neq i^*} \frac{L \log(T)}{d^*(\mu_i) \Delta_{\mu, i}}}_{\text{roughly UCB regret}} \Big).
\end{equation*}
% L is the Lipschitz constant. 
\end{conjecture}

% \begin{assumption}
% Arm $i$ knows their own value $\mu_i$ as well as the other arms' values $\mu_j$ with $j \neq i$. 
% \end{assumption}



\newpage 


% \begin{equation}
%     u_i (M, d_1, \dots, d_k) = \E \left[ \sum_{t = 1}^T \mathbb{I}(i_t = i) d_{i_t} \mu_{i_t} - m_i(\mathcal{H}_i^T) \right]
% \end{equation}


\subsection{Useful Definitions} 
Let $d_{-i} = (d_1, \dots, d_{i-1}, d_{i+1}, \dots, d_k)$ denote the strategies of all arms other than $i$. We write $M$ for a mechanism consisting of a selection rule $\pi$ and a payment rule $m$.    

\begin{definition}[Nash Equilibrium] 
We say that the strategies $(d_1, \dots, d_k)$ form a Nash equilibrium under mechanism $M$ if for all $i \in [k]$ and any deviating strategy $d_i^\prime$ of arm $i$, we have
\begin{equation*}
    u_i(M, d_i, d_{-i}) \geq u_i(M, d_i^\prime, d_{-i}).
\end{equation*}
\end{definition}

In addition, the concept of dominating strategies will be useful.  
\begin{definition}[Dominating Strategies]
We say that strategy $d_i$ is dominating under mechanism $M$ if for any deviating strategy $d_i^\prime$ and \emph{any} strategies of the other arms $d_{-i}$, we have
\begin{equation*}
    u_i(M, d_i, d_{-i}) \geq u_i(M, d_i^\prime, d_{-i}). 
\end{equation*}
We say that arms are in a \emph{dominated strategy equilibrium} if every arms plays a dominating strategy (given that it exists). 
\end{definition}


\begin{definition}
We say that the mechanism $M$ is $\varepsilon$-truthful if there exists a Nash equilibrium $(d_1, \dots, d_k)$ under $M$ such that $d_i \in [\mu_i-\varepsilon, \mu_i+\varepsilon]$ for all $i \in [k]$. 

We say that the mechanism $M$ is strongly-$\varepsilon$-truthful if there exists a dominated strategy equilibrium $(d_1, \dots, d_k)$ under $M$ such that $d_i \in [\mu_i - \varepsilon, \mu_i + \varepsilon]$ for all $i \in [k]$.  
\end{definition}



\section{Towards Question 1: Selection Rule Only} 
We here consider mechanisms that consist only of a selection rule, i.e.\ $m_i = 0$ for all $i$. 

Intuitively, a mechanism that incentives truthful market values must be able to make "credible threats" to arms. However, since the marketing values and follow-up rewards are unknown to the RS, we may expect statistical limitations to the credibility of such threats. 
\begin{lemma}[Unproven Claim]
There is no selection rule such that there exists a Nash equilibrium such that $d_i < \mu_i + \sqrt{\frac{K\log(T)}{T}}$ for all $i \in [k]$. 
\end{lemma}
\begin{proofsketch} 
Roughly speaking, when we select every arm $T/K$ many times, we can at best establish confidence intervals with radius $\sqrt{\frac{K\log(1/\delta)}{T}}$ with probability $1-\delta$ (ignoring constant factors and $\log \log$ terms). Hence, if arms play $d_i = \mu_i + \sqrt{\frac{K\log(1/\delta)}{T}}$, we cannot confidently assert that $d_i > \mu_i$. (Disclaimer: This is by far not a proper proof!)
\end{proofsketch}


Let us reformulate the social welfare objective slightly and define the social welfare regret of some selection rule, denoted $\pi$, as
\begin{align}
    R_T(\pi) = \E_{\pi} \left[ \sum_{t=1}^T d_{i_t} \mu_{i_t} - \max_i d_i \mu_i \right]
\end{align} 
Here, the expectation is taken over the algorithm's selection and the agents' strategies ($d_1, \dots, d_k$) given $\pi$. Note that we removed the penalty term and thus expect a standard MAB algorithm such as UCB to achieve low regret. This intuition can be seen to hold true: 
\begin{lemma} 
Let the selection rule $\pi$ be given by an instance of UCB with rewards/observations $c_{i_t} r_{i_t}$.
\begin{enumerate}
    \item[(1)] Under UCB, the strategy $d_i = 1$ is dominating for all arms $i\in [k]$.  
    \item[(2)] We have $R_T(\pi) = O(\sum_{i: \Delta_i > 0} \frac{\log(T)}{\Delta_i})$ with $\Delta_i = \max_j \mu_j - \mu_i$. 
\end{enumerate}
\end{lemma} 
\begin{proofsketch}
(1) follows from the fact that $d_i \mu_i$ is increasing in $d_i$ and that the expected number of times arm $i$ is played by UCB also increases with $d_i$. 

(2) follows directly from (1): If every arm plays $d_i = 1$, then we find ourselves in a classical stochastic MAB problem with observations $r_{i_t}$ and means $\mu_1, \dots, \mu_k$.
\end{proofsketch} 

This comes to no surprise as we do not penalize agents for deviating from $\mu_i$. More interesting is the question whether there exists a selection rule that achieves low regret \emph{and} is $\varepsilon$-truthful. 



\begin{algorithm}[H]
\caption{Truthful Successive Elimination}
% \caption{Playing Optimistic Nash}
\label{algorithm}
\begin{algorithmic}[1]
\STATE \textbf{input} $\delta > 0$, $\varepsilon > 0$ 
\STATE \textbf{initialize} $\mathcal{A} = [K]$
\FOR{$t \leq K \left\lceil {\log(1/\delta)}/{\varepsilon^2}\right\rceil$}
\STATE Play $i \in \argmin_{i \in \mathcal{A}} n^{t-1}_i$
\IF{$\lcb_t(d_i) > \ucb_t(\mu_i)$}
\STATE Remove $i$ from $\mathcal{A}$
\ENDIF
\ENDFOR
\FOR{$t > K \left\lceil {\log(1/\delta)}/{\varepsilon^2} \right\rceil$}
\STATE Play $i \in \argmin_{i\in \mathcal{A}} n^{t-1}_i$
\IF{$\exists j \in [K] \colon \ucb_t(\mu_i) < \lcb_t(\mu_j)$}
\STATE Remove $i$ from $\mathcal{A}$
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm} 

\begin{lemma}
Let $\delta = 1/T^2$ and $\varepsilon > \sqrt{\frac{K \log(T)}{T}}$ in Algorithm~1. It holds that:
\begin{enumerate}
    \item[(1)] For every agent $i$, the strategy $d_i = \mu_i + \varepsilon$ is dominating (in expectation) under Algorithm 1.  
    \item[(2)] The regret of Algorithm 1 is bounded as $O\left( \frac{K\log(T)}{\varepsilon^2} + \sum_{i : \Delta^\varepsilon_i > 0} \frac{\log(T)}{\Delta^\varepsilon_i} \right)$, where $\Delta^\varepsilon_i := \max_{j} \mu_j (\mu_j + \varepsilon) - \mu_i (\mu_i+\varepsilon)$. 
\end{enumerate}
The optimality gap $\Delta_i^\varepsilon$ can be understood as the best possible expected return per round when agents are at least $\varepsilon$-truthful versus the return of selecting agent $i$.  
\end{lemma}
\begin{proofsketch}
(1): For a given strategy $d_i > \mu_i$ of agent $i$, we need order $\frac{1}{(d_i - \mu_i)^2}$ many samples to distinguish $d_i$ from $\mu_i$, i.e.\ $\lcb_t(d_i) > \ucb_t(\mu_i)$. In Algorithm 1, the expected number of times we selected agent $i$ up to round $t= K \lceil \log(1/\delta) / \varepsilon^2 \rceil$ is then given by 
\begin{align*}
    n_i^t = \min \left\{ \left\lceil \frac{\log(1/\delta)}{(d_i-\mu_i)^2} \right\rceil, \left\lceil \frac{\log(1/\delta)}{\varepsilon^2} \right\rceil \right\},
\end{align*}
which is strictly increasing as $d_i \to \mu_i + \varepsilon$. In turn, $u_i(M, d_1, \dots, d_k) = \E[n_i^t] d_i \mu_i$ is increasing as $d_i \to 1$ for \emph{fixed} $n_i^t$. Hence, the strategy $d_i = \mu_i + \varepsilon$ is dominating until round $t$. ... 

(2): This bound is just the sum of the regret we suffer in the first and second part of the algorithm. 
\end{proofsketch}


\begin{remark} There are at least two intuitive extensions to the model:
\begin{enumerate}
    \item \textbf{Adaptive Marketing Values.} Instead of arms deciding on their marketing value $d_i$ at the very beginning of the game, we can allow the arms to choose the marketing value adaptively every round, i.e.\ in round $t$ arm $i$ decides on marketing value $d^t_i$. 
    \item \textbf{Multi-Slot Selection.} Instead of selecting a single item $i_t$ at time $t$, we instead must select a subset $s_t \subseteq [k]$ and arm $i \in s_t$ is clicked with probability $\frac{d_i}{\sum_{j \in s_t} d_j}$. This might introduce more competition between the arms.  
\end{enumerate}
\end{remark}


==> sections/old_notes/old_proofs.tex <==

\section{Old Proof Notes}
\subsection{Proof of Theorem~\ref{theorem:NE_characterization}}
\cdcomment{The use of both $d$ and $\s(\mu)$ is confusing. Is $d(\mu) = s^*(\mu)$?} \tkb{I changed notation from $d$ to $s$ at some point and forgot to change it here.}
We need the following technical lemma that gives an upper bound on the stopping time $\tau(\s, \mu)$, which is formally defined below. 
\begin{lemma}\label{lemma:stopping_time_upper_bound}
Let $X_1(\s), X_2(\s), \dots$ be i.i.d.\ $\mathrm{Bern}(\s)$-distributed r.v.\ with $d \in (0,1]$. Let $Y_1(\mu), Y_2(\mu), \dots$ be i.i.d.\ sub-Gaussian r.v.\ with mean $\mu\in[0,1]$.   
Denote their empirical means by $\hat X_n(\s) := \frac{1}{n} \sum_{k=1}^n X_k(\s)$ and $\hat Y_n(\mu) := \frac{1}{n} \sum_{k=1}^n Y_k(\mu)$, respectively. Let $N_{n, d}\sim \mathrm{Bin}(n, d)$ and $\alpha_n := \sqrt{\log(1/\delta) / n}$ for $\delta\in (0,1)$. Define the stopping time: 
\begin{align*}
    \tau(\s, \mu) := \min \left\{n \in \mathbb{N} \colon \hat X_n(\s) - \alpha_n(\delta) > \max_{Y \in [\hat Y_N(\mu) - \alpha_N(\delta), \hat Y_N(\mu)+\alpha_N(\delta)]} \s(Y)\right\}.  
\end{align*}
% its clipped version $\tau'(\s, \mu) := \tau(\s, \mu) \wedge T$ with $T \in \mathbb{N}$. 
Let $T \in \mathbb{N}$. There exist constants $c_1, c_2 > 0$ such that with probability $1-\delta$ 
\begin{align*}
    \tau(\s, \mu) \leq c_1\frac{H^2 \log(1/\delta)}{\s(\s-\s(\mu))^2} \quad \text{ and } \quad     \E[\tau(\s, \mu) \wedge T] \leq c_2 \frac{ H^2 \log(T)}{\s(\s-\s(\mu))^2}.
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:stopping_time_upper_bound}]
Fix $d, \mu \in [0,1]$ and $\delta \in (0,1)$. When clear from the context, we write $\hat X_n = \hat X_n(\s)$, $\hat Y_N = \hat Y_N(\mu)$, $N = N_{n, d}$ and $\alpha_n (\delta) = \alpha_n$. Recall that $\s(\mu)$ is assumed to be $H$-Lipschitz. We then have 
\begin{align*}
    \max_{Y \in [\hat Y_N - \alpha_N, \hat Y_N + \alpha_N]} \s(Y) \leq \s(\hat Y_N) + H \alpha_N ,
\end{align*}
so that for $\tilde \tau(\s, \mu) := \min \{ n\in \mathbb{N} \colon \hat X_n(\s) - \alpha_n(\delta) > \s(\hat Y_N(\mu)) + H \alpha_N\}$ it holds that $\tau(\s, \mu) \leq \tilde \tau (\s, \mu)$. 
For $\tilde \tau$ to stop, we need to reach a time $n\in \mathbb{N}$ such that 
\begin{align}\label{eq:stopping_time_sufficient}
    \hat X_n(\s) - \s(\hat Y_N(\mu)) \geq \alpha_n(\delta) + H \alpha_N(\delta). 
\end{align}
% cd: OK
\cdcomment{In the lemma statement you write $N_{n,d}$ which I guess you later abberviate to $N$? Then of course $N \leq n$, but notational inconsistencies confuse people quickly}
By merit of Hoeffding's inequality, we know that with probability $1-\delta$, $|\hat X_n(\s) - d| \leq \alpha_n(\delta)$, and using the Lipschitzness of $\s(\mu)$ (conditional on $N$): $|\s(\hat Y_N(\mu)) - \s(\mu)| \leq H | \hat Y_N(\mu) - \mu| \leq H \alpha_N(\delta)$. This implies $\hat X_n(\s) - \s(\hat Y_N(\mu)) \geq (\s - \s(\mu)) - (\alpha_n(\delta) + H \alpha_N(\delta))$. 
Using that $\alpha_n(\delta) \leq \alpha_N(\delta)$, it then follows that for a time $n$ as in \eqref{eq:stopping_time_sufficient} it is sufficient to ensure 
\begin{align*}
    d- \s(\mu) \geq 2(1+ H) \alpha_N(\delta).   
\end{align*}
Hence, we get that $\hat X_n (\s) - \s(\hat Y_N(\mu)) \geq \alpha_n(\delta) + H \alpha_N(\delta)$ with at least probability $1-\delta$ for $N \geq \frac{c H^2 \log(1/\delta)}{(\s-\s(\mu))^2}$. Now, using Chernoff's inequality, we have again with probability $1-\delta$ that $|N - nd| \leq \sqrt{n \log(1/\delta)}$ and thus $N \geq nd - \sqrt{n\log(1/\delta)}$. Hence, we find that for $N \geq \frac{c H^2 \log(1/\delta)}{(\s- \s(\mu))^2}$ to hold with probability $1-\delta$, we can choose $n = O\big(\frac{H^2 \log(1/\delta)}{\s(\s-\s(\mu))^2} \big)$. This shows the high probability bound on $\tau(\s, \mu)$. 
To obtain the bound on $\E[\tau(\s, \mu) \wedge T]$, note that for $\delta = 1/T^2$, we obtain for some $c_2 > 0$
\begin{align*}
    \E [\tau(\s, \mu) \wedge T] \leq (1-1/T^2) \frac{c_1 H^2 \log(1/\delta)}{\s(\s-\s(\mu))^2} + T/T^2 \leq c_2 \frac{H^2 \log(1/\delta)}{\s(\s-\s(\mu))^2} . 
\end{align*}
\end{proof} 

We are now ready to prove Theorem~\ref{theorem:NE_characterization}. 

\begin{proof}[Proof of Theorem~\ref{theorem:NE_characterization}]
Let $\bs=(\s_1,\dots,\s_K)$ denote any Nash equilibrium under UCB-S. We write $\E_\bs [n_t(i)]$ for the expected number of times arm $i$ is selected up to round $t$ under strategies $\bs = (\s_1, \dots, \s_K)$ and mechanism UCB-S. 
To analyse the Nash equilibrium, we will use the following trick that will allow us to introduce $\E[\tau(\s_i, \mu_i)]$ into the surplus function. 
\begin{claim}\label{claim:min} 
$\E_\bs [ n_T(i)] \leq 2 \E[\tau(\s_i, \mu_i)]$ for all $i \in [K]$.  % \wedge \E_\bs [n_T(i)]$.  
\end{claim}
\begin{proof}[{Proof of Claim~\ref{claim:min}.}]
The total number of times arm $i$ is played under UCB-S is determined by the screening rule and the UCB selection rule. When the screening rule is triggered for some arm $i$, this arm is not being played anymore with high probability. We can trivially bound this probability by $1/2$. Hence, it follows from monotonicity that $\E_\bs[n_T(i)] \leq 2 \E[\tau(\s_i, \mu_i)]$.\footnote{Note that $n_T(i)$ and $\tau(\s_i, \mu_i)$ can be expressed as stopping times (which satisfy $n_T(i) \leq 2 \tau(\s_i, \mu_i)$ always). \cdcomment{This is not obvious.}}
\end{proof}


Based on Claim~\ref{claim:min} we express the surplus of arm $i$ under the Nash equilibrium $\bs$ as
\begin{align}\label{eq:surplus_samples}
    S_i (\s_i, \s_{-i}) 
    = \E_\bs [n_T(i)] \s_i \nu_i 
    = \big(\E[\tau(\s_i, \mu_i)] \wedge \E_\bs [n_T(i)]\big)  \s_i \nu_i. 
\end{align} 
% We have established at an earlier step that $\s_i \geq \s(\mu_i)(1-1/T^2)$. 
To derive an upper bound on $\s_i$, we express arm $i$'s Nash equilibrium strategy as $\s_{i} := \s(\mu_{i}) + \varepsilon$ for some $\varepsilon > 0$. Lemma~\ref{lemma:stopping_time_upper_bound} gives us an upper bound on $\E_\bs [\tau(\s(\mu_i)+\varepsilon, \mu_i)]$, which when plugged into equation \eqref{eq:surplus_samples} yields
\begin{align}\label{eq:surplus_plugge\s_in}
    S_{i} (\s(\mu_{i}) + \varepsilon, \s_{-i}) & = \Big( c \frac{H^2 \log(T)}{\s(\mu_i) \varepsilon^2} \wedge \E_{\bs}[n_T(i)] \Big) (\s(\mu_{i}) + \varepsilon) \nu_{i}, 
\end{align}
where we used that $\s_i - \s(\mu_i) = \varepsilon$ and $\s(\mu_i) \leq \s(\mu_i) + \varepsilon$. Note that it is valid to plug in an upper bound for $\E[\tau(\s_i,\mu_i)]$, since $\E_\bs [n_T(i)] \leq \E[\tau(\s_i, \mu_i)]$ by Claim~\ref{claim:min}. \cdcomment{The 2 is missing}
We observe that the surplus as a function of $\varepsilon$ is monotonically increasing for $\varepsilon  < \sqrt{c H^2 \log(T)/ \s(\mu_i) \E_{\bs}[n_T(i)]}$ and otherwise monotonically decreasing. 

Note that $\E_{\bs} [n_T(i)]$ itself depends on $\varepsilon$ through $\s_i := \s(\mu_i) + \varepsilon$. To show (i), we then aim to derive a lower bound on $\E_\bs [n_T(i^*)]$ for any optimal arm $i^* \in [K^*]$ using only the fact that $\bs$ is a Nash equilibrium without arguing about $\varepsilon$ directly. This then leads to a characterization of $\varepsilon$. 
%\footnote{Note that such a lower bound is trivial for any low-regret bandit algorithm. However, we have not yet analysed UCB-S.}


\begin{claim}\label{claim:lower_boun\s_nT}
If $\bs$ is a Nash equilibrium, then $\E_\bs [n_T(i^*)] \geq \s(\mu_{i^*})T/K$ for any optimal arm $i^*\in [K^*]$. 
% \textcolor{purple}{I'm very confident that the $\s(\mu_{i^*})$ factor can be removed.}
\end{claim}
\begin{proof}[{Proof of Claim~\ref{claim:lower_boun\s_nT}.}]
Recall that $\mathbb{P}(i^* \in A_t \forall t\in [T] \mid \s(\mu_{i^*})) \geq 1-1/T^2$. Then, under strategy $\s(\mu_{i^*})$, we have $\E [n_T(i^*) \mid (\s(\mu_{i^*}), d'_{-i^*})] \geq T/K$ for $T$ sufficiently large and for all possible opponent strategies $d'_{-i^*}$.\footnote{This can be checked in detail using that $\E[n_T(i^*) \mid \mathcal{E}_{i^*}] \geq \E[n_T(i^*) \mid \mathcal{E}_{i^*}, \mathcal{E}_i]$ for all $i\neq i^*$ and a simple symmetry argument.}
Now, since $\bs = (\s_1, \dots, \s_K)$ is a Nash equilibrium, we have $S_{i^*}(\s_{i^*}, \s_{-i^*}) \geq S_{i^*} (\s(\mu_{i^*}), \s_{-i^*})$ and it therefore must hold that
\begin{align*}
    \E [n_T(i^*) \mid {(\s_{i^*}, \s_{-i^*})}] \geq \s_{i^*}  \E [n_T(i^*) \mid {(\s_{i^*}, \s_{-i^*})}] \geq \s(\mu_{i^*}) \E [n_T(i^*) \mid  {(\s(\mu_{i^*}), \s_{-i^*})}] \geq \s(\mu_{i^*}) T/K.  
\end{align*}
\end{proof} 
Then, due to the monotonicity of the surplus function in \eqref{eq:surplus_plugge\s_in}, the upper bound on $\E_\bs[n_T(i^*)]$ implies that $\varepsilon \leq \sqrt{c H^2 K \log(T) / \s(\mu_{i^*})^2 T}$ with $\s_{i^*} := \s(\mu_{i^*}) + \varepsilon$. 


\end{proof}

To characterize the Nash equilibrium strategies of suboptimal arms under UCB-S, we must establish lower bounds on $\E_\bs [n_T(i)]$. The following lemma is a consequence of a well-known result stating that any low-regret algorithm in the minimax sense, must play each suboptimal arm $i$ at least order $\log(T)/ \Delta_i^2$ many times. 
\begin{lemma}
    Under UCB-S, for any $i \not \in [K^*]$ and any $\bs \in \NE(\ucbs)$ and $\bs \in \supp(\bs)$, there exists a universal constant $c \geq 0$ such that
    \begin{align*}
        \E [n_T(i) \mid (\s_i, \sigma_{-i})] \geq \frac{c \log(T)}{\s_i \Delta_i^2}. 
    \end{align*}
    A more detailed expression of the constant factor $c$ can be found in, e.g., \cite{lattimore2020bandit}. 
\end{lemma}
\begin{proof}
    A standard result from the instance-dependent lower bound analysis of the multi-armed bandit problem (e.g., Lemma 16.2 in \cite{lattimore2020bandit}) states that any algorithm that suffers sublinear minimax regret, must play each arm order $\log(T)/ \Delta_i^2$ many times, where $\Delta_i$ is the optimality gap.\footnote{Note that this is under the assumption of sub-Gaussian reward distributions. Otherwise, the denominator can be expressed using the KL-divergence of the respective reward distributions.} Of course, the traditional UCB algorithm is one such algorithm.  
    
    Now, let $\mathcal{E}_i = \{ i \in A_t \, \forall t \in [T]\}$ and recall that $\P( \mathcal{E}_i \mid \s(\mu_i)) \geq 1-1/T^2$. Our UCB-S mechanism deploys a UCB-type selection rule so that $\E[n_T(\mu, i) \mid (\s(\mu_i), \sigma_{-i})] \geq c \log(T) / \Delta_i^2$ holds for some universal constant $c > 0$.\footnote{We here used that $\P(\mathcal{E}_i \mid \s(\mu_i)) \geq 1 - 1/T^2$, which can again be always lower bounded by, e.g., $1/4$ when $T \geq 2$.} Since $\E [n_T(\mu, i) \mid (\s(\mu_i), \sigma_{-i})] = \s(\mu_i) \E [n_T(i) \mid (\s(\mu_i), \sigma_{-i})]$, 
    it then follows that $$\E [n_T(i) \mid (\s(\mu_i), \sigma_{-i})] \geq \frac{c \log(T)}{\s(\mu_i) \Delta_i^2}.$$ 
    Since $\s_i$ has to be a best-response to $\sigma_{-i}$, we get that
    \begin{align*}
        \s_i \E[n_T(i) \mid (\s_i, \sigma_{-i})] \geq \s(\mu_i) \E [ n_T(i) \mid (\s(\mu_i), \sigma_{-i})] \geq \frac{c\log(T)}{\Delta_i^2}, 
    \end{align*}
    which implies $\E [n_T(i) \mid (\s_i, \sigma_{-i})] \geq \frac{c\log(T)}{\s_i \Delta_i}$. 
\end{proof}



\newpage 


\newpage 


% \begin{lemma}
%     Under any Nash equilibrium $\bsigma \in \NE(\ucbs)$, we have 
%     \begin{align*}
%         \E_{\bsigma}[\tau_{i^*}] \geq \E_{\bsigma} [\tau_i].
%     \end{align*}
% \end{lemma}

\begin{lemma} 
    % Let $\nu_{i^*} := \min\{ t \in \mathbb{N} \colon i^* \not\in A_t\}$. 
    Let $\nu := \min\{ t \in \mathbb{N} \colon A_t = \emptyset \}$. 
    Under any Nash equilibrium $\bsigma \in \NE(\ucbs)$ for any $\delta> 0$ it holds that with probability at least $1-\delta$: 
    \begin{align*}
        \nu >  T- O\Big(\frac{\sqrt{KT}}{1-\delta}\Big). 
    \end{align*}
\end{lemma}
\begin{proof} 
    % W.l.o.g.\ let $i^* := \argmax_{i} \mu_i$ be unique, i.e., $[K^*] = \{i^*\}$. The proof follows analogously for non-unique optimal arms by defining $i^*$ to be the last arm to be eliminated. 
    We prove the statement by contradiction, showing that no Nash equilibrium could allow for the converse to happen due to $\s_{i^*}$ having to be a best response to $\sigma_{-i^*}$, where $i^*$ is an optimal arm.  
    Suppose there exists $\delta > 0$ such that with probability $1-\delta$ under $\bsigma$, we have $$ \nu < T - \omega\Big(\frac{\sqrt{KT}}{1-\delta}\Big).$$   
    Consider an arm $i^*$ and for any $\s_{i^*} \in \supp(\sigma_{i^*})$ the strategy profile $(\s_{i^*}, \sigma_{-i^*})$. For convenience, we omit the subscript $\sigma_{-i^*}$ in the following. Now, recall that $$\E_{\s_{i^*}}[\tau_{i^*}] \geq \E_{\s_{i^*}}[n_T(i^*)] \geq T/K. $$
    
    %Let $\varepsilon := \s_{i^*} - \s^*(\mu_{i^*})$. 
    Based on the above we get that $\s_{i^*} - \s^*(\mu_{i^*}) = O({1}/{\sqrt{\E_{\s_{i^*}}[n_T(i^*)]}}) = O(\sqrt{K/T})$. Now, for $\s'_{i^*} := \s^*(\mu_{i^*}) + \frac{s_{i^*} - \s^*(\mu_{i^*})}{\sqrt{K}}$, we get that $\E_{\s'_{i^*}}[\tau_{i^*}] \geq T$. As a result, since  $\E_{\s'_{i^*}}[n_T(i^*)] \geq \E_{\s_{i^*}}[n_T(i^*)] + \omega(\sqrt{KT})$. Then,
    \begin{align*}
        \U_{i^*}(\s'_{i^*}, \sigma_{-i^*}) & \geq \left( \E_{\s_{i^*}}[n_T(i^*)] + \omega(\sqrt{KT}) \right) \s'_{i^*} \\ 
        & = \left( \E_{\s_{i^*}}[n_T(i^*)] + \omega(\sqrt{KT}) \right) \left(\s^*(\mu_{i^*}) + \frac{\s_{i^*} - \s^*(\mu_{i^*})}{\sqrt{K}} \right) \\ 
        & = \left( \E_{\s_{i^*}}[n_T(i^*)] + \omega(\sqrt{KT}) \right)  \left(\s^*(\mu_{i^*}) + O \Big(\frac{1}{\sqrt{K \E_{\s_{i^*}} [n_T(i^*)] }}\Big) \right) \\ 
        & \geq \E_{\s_{i^*}}[n_T(i^*)] \s^*(\mu_{i^*}) + \omega(\sqrt{KT}) \s^*(\mu_{i^*}) + O\Big( \sqrt{\frac{\E_{\s_{i^*} [n_T(i^*)]}}{K}} \Big) + O(1) \\ 
        & > \E_{\s_{i^*}}[n_T(i^*)] \s^*(\mu_{i^*}) + O\Big(\sqrt{\E_{\s_{i^*}}[n_T(i^*)]}\Big) \\[0.2em]
        & \geq \E_{\s_{i^*}}[n_T(i^*)] \s_{i^*} \\[0.5em]
        & = \U_{i^*} (\s_{i^*}, \sigma_{-i^*}),   
    \end{align*}
    where we used that $\E_{s_{i^*}} [n_T(i^*)] \leq T$ by definition. Hence, $\s'_{i^*}$ is a strictly better response to $\sigma_{-i^*}$ than $\s_{i^*}$, which is a contradiction. \tkb{It's possible to account for the $\omega(\sqrt{KT}) / K = \omega(\sqrt{T /K})$ allocations an arm receives after $\nu$, since $\omega(\sqrt{T/K}) \leq \s^*(\mu_{i^*}) \omega(\sqrt{K T})$. }
\end{proof}



\begin{lemma}
    For every $i^* \in [K^*]$ and every $\s_{-i^*} \in [0,1]^{K-1}$, the number of times $i^*$ is selected by $\ucbs$, i.e., $\E_{(\s_{i^*}, \s_{-i^*})}[n_{T}(i^*)]$, monotonically decreases as $\s_{i^*}$ increases on $[\s^*(\mu_{i^*}), 1]$.   
\end{lemma}
\newpage 




\input{sections/motivation_figure}



==> sections/setting-backup.tex <==

\hf{The following is a backup of the original version. }

We assume that the mechanism $M$ is fixed ahead of time and shared with the agents. With knowledge of $M$, the agents get to decide on their strategies $(\s_1, \dots, \s_K) \in [0,1]^K$ through which the agents can influence the click probability of users. More precisely, every round $t$, the mechanism chooses to allocate an impression to some agent $i_t \in [K]$ upon which the user clicks $i_t$ with probability $s_{i_t}$ after which a post-click reward with mean $\mu_{i_t} \in [0,1]$ is observed. The interaction is specified below:


% We consider a set of $K$ strategic agents,  $ [K] := \{ 1, . . . , K\}$, that interact with users and a principal through an online mechanism $M$.  We assume that the mechanism $M$ is fixed ahead of time and shared with the agents. With knowledge of $M$, the agents get to decide on their strategies $(\s_1, \dots, \s_K) \in [0,1]^K$ through which the agents can influence the click probability of users. More precisely, every round $t$, the mechanism chooses to allocate an impression to some agent $i_t \in [K]$ upon which the user clicks $i_t$ with probability $s_{i_t}$ after which a post-click reward with mean $\mu_{i_t} \in [0,1]$ is observed. The interaction is specified below:


% We assume that each agent $i$ has a true post-click reward $\mu_i \in [0,1]$, which is privately known to agent~$i$. In addition, we assume that each agent~$i$ is aware of the largest value (not index) $\mu_* := \max_{i\in [K]} \mu_i$. We specify the interaction between the agents and the principal as follows: 




The following two assumptions specify the information available to the principal and the agents. 

\begin{assumption}
    The mechanism $M$ does not see the agent strategies $s_1, \dots, s_K$ in advance, but only observes the click-event $c_{t, i_t}$ in round $t$. Similarly, the mechanism does not know the mean post-click rewards $\mu_1, \dots, \mu_K$ in advance, but only observes the realized post-click reward $r_{t, i_t}$ in round $t$.  
\end{assumption} 


\begin{assumption}
    Every agent $i\in [K]$ has private knowledge of their mean post-click reward $\mu_i \in [0,1]$ and also knows the maximal value (not index) $\mu^* := \max_{i \in [K]} \mu_i$.
\end{assumption}



\subsection{Agent's Utility and Nash Equilibrium of the Agents}
Let $\s_{-i}$ denote the $K-1$ strategies of all agents except $i$. We assume that each agent $i$ has a private value-per-click $\nu_i > 0$ that is only known to agent $i$. \hf{I think this is not important since it will not affect agent $i$'s optimization.} \tkb{Yes, we could remove $\nu_i$ all together and just consider $\E[n_T(i)] \s_i$, i.e., allocations x click-rate, as the objective.} \hf{Actually, can $\nu_i$ also depends on $s_i $ (i.e., more aggressive promotion may harm the value per click)? Can we work out this more general case as well? So the utility will be $\sum_{t=1}^T \ind{\{i_t = i\}} \s_i \nu_i (\s_i)$.  } \tkb{I thought about this ("a general theory" not only for this setting but more generally for mechanism design + statistical estimation) a while back. It is quite important how $\nu_i(\s_i)$ behaves, i.e., how "dishonesty" of the agent is rewarded in said agent's utility. For example, if $\nu_i(\s_i)$ is increasing exponentially with $\s_i$ the "threat of elimination/detection" is not scary compared to the reward gained through $\nu_i(\s_i)$ (when we estimate a quantity we typically have necessary sample complexity $\Theta(1/\text{dishonesty}^2)$) As the mechanism designer we then in some sense lose control over the agents. However, I haven't fully understood how a function $\nu_i(\s_i)$ would really impact the incentive design, so I don't know I'm afraid.} \hf{I see. Let's leave this as an open question in the conclusion section then. THis is indeed a nice generalization though. } In a special case, this value could equal the post-click value, i.e., $\nu_i = \mu_i$, or simply $\nu_i = 1$. Each agent's objective is to maximize their cumulative payoff which is determined by the number of impressions allocated to them as well as the click probability $s_i$ and value-per-click $\nu_i$. 
%Let $n_T(i)$ be the number of times the mechanism selects agent $i$ over $T$ rounds. 
The \emph{expected utility} of agent $i$ under mechanism $M$ and strategies $(\s_i, \s_{-i})$ is then given by
\begin{equation}
    \U_i(M, \s_i, \s_{-i}) := 
    \E_M \left[ \sum_{t=1}^T \ind{\{i_t = i\}} \s_i \nu_i  \right] % = \E_M [n_T(i)]  \s_{i} \nu_{i} ,
\end{equation}
where the expectation is taken over the mechanism's decisions, which themselves could depend on the environment's randomness as well as the agent strategies. Let $\Sigma$ denote the set of probability measures over $[0,1]$. For a mixed strategy profile $\bsigma = (\sigma_i, \sigma_{-i}) \in \Sigma^K$, i.e., a distribution over pure strategies $\bs \in [0,1]^K$, the surplus under mechanism $M$ is defined as $S_i (M, \sigma_i, \sigma_{-i}) := \E_{\bs \sim \bsigma} [S_i(M, \s_i, \s_{-i})]$. 


We assume that the agents play a Nash equilibrium of the game induced by the algorithm $M$ defined as follows:
\begin{definition}[Nash Equilibrium]
We say that the strategies $\bsigma = (\sigma_1, \dots, \sigma_K)$ are a Nash equilibrium under mechanism $M$ if $\U_i (M, \sigma_i, \sigma_{-i}) \geq \U_i (M, \sigma^\prime_i, \sigma_{-i})$ for all $i \in [K]$ and strategies $\sigma^\prime_i \in \Sigma$. 
\end{definition} 



If the mixed strategy profile $\bsigma \in \Sigma^K$ equals a pure strategy profile $\bs \in [0,1]^K$ with probability one, the Nash equilibrium is said to be in pure strategies. 
Let $\mathrm{NE}(M):=\{\bsigma \in \Sigma^K \colon \bsigma \text{ is a NE under } M\}$ denote the set of all (possibly mixed) Nash equilibria for the agents under mechanism $M$.



% \begin{definition}[$\varepsilon$-Nash Equilibrium]
% For $\varepsilon >0$, we say that strategies $\bsigma = (\sigma_1, \dots, \sigma_K)$ are an $\varepsilon$-Nash equilibrium under mechanism $M$ if $\U_i(M, \sigma_i , \sigma_{-i}) \geq \U_i(M, \sigma^\prime_i, \sigma_{-i}) - \varepsilon$ for all $i \in [K]$ and $\sigma^\prime_i \in \Sigma$. We denote the set of all $\varepsilon$-Nash equilibria under $M$ as $\NE_\varepsilon := \{ \bsigma \in \Sigma^K \colon \bsigma \text{ is } \varepsilon\text{-NE under } M\}$. 
% \end{definition}


\begin{remark}[Existence of Nash Equilibrium]
In general, a game with continuous strategy space, e.g.\ $[0,1]$, may not posses a Nash equilibrium. In our situation, this is also the case and not every mechanism necessarily induces a game with a Nash equilibrium for the agents. However, we will prove the existence of a Nash equilibrium for all considered algorithms by either stating the Nash strategies explicitly or proving the existence in a more abstract way. 
%To this end, we will prove the existence of a Nash equilibrium for the agents under all mechanisms considered hereafter. 
% Until then, let us not be further bothered by the question of existence.  
\end{remark}

% \textcolor{purple}{\textbf{Note:} What should we call $\s$ and $\mu$? $\s$ = strategies, marketing values? $\mu$ = post-click feedback, true value, post-click value?}


\subsection{Principal's Utility and Strategic Regret} 

We denote the principal's utility of selecting an agent $i$ with marketing value $\s_i$ and post-click value $\mu_i$ by $u(\s_i, \mu_i)$. \hf{why not $u_i(\s_i, r_i)$? Would this generalization also work?} \tkb{Recall that $r_i$ are the observed rewards, which have mean $\mu_i$. If we define the utility for the random variables $r_i$ instead of the mean $\mu_i$ the problem (I think) is that in general $\E [u(\s_i, r_i)] \neq u(\s_i, \mu_i)$. Note that the utility is currently defined w.r.t.\ the mean values $\s_i$ and $\mu_i$.}  \cdcomment{Yes, $u$ is not a linear function of rewards.} \hf{I was thinking of $\bar{u}(f_i, s_i) = \mathbb{E}_{r_i \sim f_i} u (r_i, s_i)$ and learn $\bar{u}(f_i, s_i)$ instead.....but maybe it is okay, let's stick with $u(\s_i, \mu_i)$ then. \tkb{That should be possible because $u$ is assumed to be Lipschitz, but I'm not absolutely sure.} However, can $u$ be $u_i$ instead? That is, different arm has different $u_i$ function?}\tkb{Yes (95\% sure), we can have different $u_i$ for arms as long as every $u_i$ satisfies the assumptions below.} An example of this is the {greedy} utility function $u(\s, \mu) = \s\mu$, which is indifferent about how much the click-rates $\s$ differ from the post-click value $\mu$. However, the principal may value consistency between the click-rates and the post-click values. This could be captured by a penalty term, e.g., for some $\lambda > 0$ consider $u(\s, \mu) = \s\mu - \lambda(\s-\mu)^2$. 
% \begin{align}\label{eq:example_u}
    % u(\s, \mu) = \s\mu - \lambda(\s-\mu)^2 .
% \end{align} 
% We will use the above utility function as a running example, 
We keep the above utility function in mind as a running example, but derive our results for a general class of functions $u$ satisfying the following regularity assumptions: \hf{Does the following assumptions  include functions like $u(s_i, \mu_i) = s_i \mu_i \times \mathbb{I} \big[ (s_i - \mu_i)^2 \leq c \big] $? Would be really nice if we can handle this style of functions.   } \tkb{I think so. Even though $u$ is not differentiable, it is Lipschitz and satisfies A1-A3 as far as I can tell. $u^*(\mu)$ is increasing and if I am not mistaken $s^*(\mu) = \min\{ \mu  + \sqrt{c}, 1\}$.}
\begin{enumerate}
    \item[\mylabel{item:a1}{(A1)}] $u \colon [0,1] \times [0,1] \to \mathbb{R}$ is $L$-Lipschitz w.r.t.\ the $\ell_1$-norm.
    \item[\mylabel{item:a2}{(A2)}] $u^*(\mu) := \max_{\s\in [0,1]} u(\s, \mu)$ is monotonically increasing. 
    \item[\mylabel{item:a3}{(A3)}] $\s^*(\mu) := \argmax_{\s\in [0,1]} u(\s, \mu)$ is $H$-Lipschitz and is bounded away from zero.
\end{enumerate}
Assumption (i) bounds the loss of selecting a suboptimal agent. 
Assumption (ii) states that agents with larger post-click rewards $\mu$ are preferred given that the agent plays the desired strategy in terms of the principal's utility $u$. 
Assumption (iii) then ensures that the optimal strategies in terms of $u$ are bounded away from zero and do not change abruptly w.r.t.\ $\mu$.\footnote{The specific range of $\s^*(\mu)$ does not matter. However, it is necessary to bound $\s^*(\mu)$ away from zero to prevent absurd cases where the principal would like every agent's click-rate to be zero.}
% Note that the running example of $u(\s,\mu) = \s\mu - \lambda(\s-\mu)^2$ is $5\lambda$-Lipschitz as well as $u^*(\mu)$ monotonically increasing and $\s^*(\mu) = (1+\frac{1}{2\lambda})\mu$ also Lipschitz. 
In the following, the function $\s^*(\mu)$ will play a central role as it describes the optimal agent strategies in terms of the principal's utility, i.e., the strategies that the principal needs to incentivize. 

\paragraph{Strategic Regret.}
The principal's goal is to maximize utility $\sum_{t=1}^T u(\s_{i_t}, \mu_{i_t})$ over $T$ rounds, which naturally depends on the agents' strategies $\bs$. For given $\mu_1, \dots, \mu_K$, the optimal utility $u(\s^*, \mu^*)$ is then achieved by $\mu^* := \max_{i \in [K]} \mu_i$ and $\s^* := \s^*(\mu^*)$.  With $u(\s^*, \mu^*)$ as a benchmark, we then define the \emph{strategic regret} of a mechanism $M$ and strategies $\bs \in [0,1]^K$ as 
\begin{equation}
    R_T(M, \bs) :=  \E \left[ \sum_{t=1}^T  u(\s^*, \mu^{*}) - u(\s_{i_t}, \mu_{i_t}) \right] .
\end{equation}
For mixed strategies $\bsigma \in \Sigma^K$, we then define the strategic regret as $R_T(M, \bsigma) := \E_{\bs \sim \bsigma} [R_T(M, \bs)]$. 

We are going to evaluate a mechanism $M$ under the Nash equilibria $\NE(M)$ it induces among the agents. Here, we can consider the the \emph{strong strategic regret} of $M$ given by the regret under the worst-case Nash equilibrium: $\max_{\bsigma \in \mathrm{NE}(M)} R_T(M, \bsigma)$, or the \emph{weak strategic regret} defined as the regret under the most favorable Nash equilibrium: $\min_{\bsigma \in \mathrm{NE}(M)} R_T(M, \bsigma)$. 

% \begin{equation}
%     R^{+}_T(M) := \max_{\bsigma \in \mathrm{NE}(M)} R_T(M, \bsigma),
% \end{equation}
% and its weak counterpart as the \emph{weak strategic regret} given by the performance under the most favorable Nash equilibrium under $M$:
% \begin{equation}
%     R^{-}_T(M) := \min_{\bsigma \in \mathrm{NE}(M)} R_T(M, \bsigma).
% \end{equation}


\subsection{Necessity of Incentive Design: Lower Bounds for Incentive-Unaware Oracles}

Importantly, to achieve low (weak or strong) strategic regret, it is insufficient to find simply find $\argmax_i \mu_i$ or $\argmax_i u(\s_i, \mu_i)$. To illustrate this, we show that even with oracle knowledge of $\mu_1, \dots, \mu_K$ and $\s_1, \dots, \s_K$ algorithms can suffer linear strategic regret if they fail to design the right incentives for the agents. 

The general class of utility functions $u$ is very broad and contains utility functions that are trivial to maximize. For example, if $u(s^*, \mu^*) - u(s, \mu) = O(1/T)$ for all $s, \mu$, any algorithm would only suffer constant regret $O(1)$. To derive meaningful lower bounds, we therefore restrict our attention to utility functions under which the loss of deviating from the maximal utility $u(\s^*, \mu^*)$ is lower bounded. We formalize this property as $u$ being locally reverse Lipschitz at $(\s^*, \mu^*)$. 
\begin{definition}[Locally Reverse Lipschitz]
The utility function $u$ is locally reverse $\smash{\tilde L}$-Lipschitz at $(s^*, \mu^*)$ if $| u(\s^*, \mu^*) - u(\s, \mu)| \geq \tilde L (| \s^*- \s | + |\mu^* - \mu |)$ for all $\s \in [0,1]$ and $\mu \in [0,1]$. 
\end{definition}

... 

\begin{proposition}\label{prop:oracles} 
Let $\mu_1, \dots, \mu_K \in [0,1]$ with unique $i^* \in \argmax_{i \in [K]} \mu_i$ and define $\Delta_i := \mu^* - \mu_i$ and $\Delta := \min_{i \neq i^*} \Delta_i$. For any utility function $u$ that satisfies \ref{item:a1}-\ref{item:a3} and is locally reverse $\smash{\tilde L}$-Lipschitz at $(\s^*, \mu^*)$ with $\s^* \leq c$ for some constant $c \in (0,1)$, 
the following hold:
\begin{enumerate}
    \item[(i)] Let $Oracle_\mu$ be the algorithm with oracle knowledge of $\mu_1, \dots, \mu_K$ that plays $i_t = \argmax_{i \in [K]} \mu_i$ in every round $t$. For all Nash equilibria $\bsigma \in \NE(Oracle_\mu)$ of the agents, the algorithm suffers regret 
    $$R_T(Oracle_\mu, \bsigma) =\Omega (\smash{\tilde L} T ). $$ 
    \item[(ii)] Let $Oracle_{\mu, \s}$ be the algorithm with oracle knowledge of $\mu_1,\dots, \mu_K$ and $\s_1, \dots, \s_K$ that plays $i_t = \argmax_{i \in [K]} u(\s_i, \mu_i)$ in every round $t$ with ties broken in favor of the larger $\mu$. For all Nash equilibria $\bsigma \in \NE(\oraclesm)$ of the agents, the algorithm suffers regret
    $$R_T(Oracle_{\mu, \s}, \bsigma) = \Omega( \Delta \smash{\tilde L} T).$$
    
    
    % \item[(iii)] Let $Oracle^\prime_{\mu, \s}$ be the algorithm with oracle knowledge of $\mu_1,\dots, \mu_K$ and $\s_1, \dots, \s_K$ that plays $i_t = \argmax_{i \in [K]} u(\s_i, \mu_i)$ in every round $t$ with ties broken uniformly. For all $\varepsilon > 0$ there exists an $\varepsilon$-Nash equilibrium $\bsigma \in \NE_\varepsilon(Oracle^\prime_{\mu, \s})$ for the agents such that $$R_T(Oracle^\prime_{\mu, \s}, \bsigma) = \Omega( \Delta \smash{\tilde L} T).$$
\end{enumerate}
\end{proposition} 
\begin{proof}[Proof Sketch] 
\textit{(i)}: We show that under the described algorithm $\s = 1$ is a strictly dominant strategy for agent $i^*$. This implies that agent $i^*$ plays $\s_{i^*} = 1$ with probability one in every Nash equilibrium under the oracle algorithm. The claimed lower bound then follows from bounding the instantaneous regret from below using $\s^*(\mu_{i^*}) \leq c$. \textit{(ii)}: Let $j^* \in \argmax_{i \neq i^*} \mu_i$. It can be seen that in any Nash equilibrium, agent $i^*$ will play the largest $\s \in [0,1]$ such that $u(\s, \mu_{i^*}) \geq u(\s_{j^*}, \mu_{j^*})$. We then show that (at least) either $\s_{i^*} = 1$ or $u(\s_{i^*}, \mu_{i^*}) = u(\s^*(\mu_{j^*}), \mu_{j^*})$. Once again this allows us to bound the instantaneous regret per round from below, which yields the claimed lower bound. %\textit{(iii)}: The subtle change that ties are broken now uniformly instead of in favor of the larger $\mu$ has the consequence that in all but a few problem instances no Nash equilibrium for the agents exists. For a given $\varepsilon > 0$ then explicitly construct a $\varepsilon$-Nash equilibrium for the agents under which the algorithm suffers regret similar \textit{(ii)}. 
\end{proof} 


\begin{remark}
    Interestingly, when the oracle algorithm from Proposition~\ref{prop:oracles}~\textit{(ii)} does not break ties in favor of the larger $\mu$ but instead uniformly at random, it can be shown that in all but a few problem instances no Nash equilibrium for the agents exists. However, for any $\varepsilon > 0$ we can explicitly construct an $\varepsilon$-Nash equilibrium for the agents under which the algorithm suffers $\Omega (\Delta \smash{\tilde L } T)$ regret. More details can be found in Appendix~X and the proof of Proposition~\ref{prop:oracles}. 
\end{remark}


% \hf{This shows the necessity of   incentive design -- this problem is beyond a pure learning question. }
